Unsupervised Deep Learning for Structured Shape Matching

We present a novel method for computing correspondences across 3D shapes using unsupervised learning. Our method computes a non-linear transformation of given descriptor functions, while optimizing for global structural properties of the resulting maps, such as their bijectivity or approximate isometry. To this end, we use the functional maps framework, and build upon the recent FMNet architecture for descriptor learning. Unlike that approach, however, we show that learning can be done in a purely \emph{unsupervised setting}, without having access to any ground truth correspondences. This results in a very general shape matching method that we call SURFMNet for Spectral Unsupervised FMNet, and which can be used to establish correspondences within 3D shape collections without any prior information. We demonstrate on a wide range of challenging benchmarks, that our approach leads to state-of-the-art results compared to the existing unsupervised methods and achieves results that are comparable even to the supervised learning techniques. Moreover, our framework is an order of magnitude faster, and does not rely on geodesic distance computation or expensive post-processing.

==> sec-bib.tex <==
\begin{thebibliography}{10}\itemsep=-1pt

\bibitem{tensorflow2015-whitepaper}
M.~Abadi, A.~Agarwal, and P.~B. et~al.
\newblock {TensorFlow}: Large-scale machine learning on heterogeneous systems,
  2015.
\newblock Software available from tensorflow.org.

\bibitem{aflalo2013spectral}
Y.~Aflalo, A.~Dubrovina, and R.~Kimmel.
\newblock Spectral generalized multi-dimensional scaling.
\newblock {\em International Journal of Computer Vision}, 118(3):380--392,
  2016.

\bibitem{scape}
D.~Anguelov, P.~Srinivasan, D.~Koller, S.~Thrun, J.~Rodgers, and J.~Davis.
\newblock {SCAPE}: {S}hape {C}ompletion and {A}nimation of {P}eople.
\newblock In {\em ACM Transactions on Graphics (TOG)}, volume~24, pages
  408--416. ACM, 2005.

\bibitem{aubry11}
M.~Aubry, U.~Schlickewei, and D.~Cremers.
\newblock The wave kernel signature: A quantum mechanical approach to shape
  analysis.
\newblock 31(4), Nov. 2011.

\bibitem{biasotti2016recent}
S.~Biasotti, A.~Cerri, A.~Bronstein, and M.~Bronstein.
\newblock Recent trends, applications, and perspectives in 3d shape similarity
  assessment.
\newblock In {\em Computer Graphics Forum}, volume~35, pages 87--119, 2016.

\bibitem{bogo2014}
F.~Bogo, J.~Romero, M.~Loper, and M.~J. Black.
\newblock {FAUST}: Dataset and evaluation for {3D} mesh registration.
\newblock In {\em Proceedings IEEE Conf. on Computer Vision and Pattern
  Recognition (CVPR)}, Piscataway, NJ, USA, June 2014. IEEE.

\bibitem{boscaini2015learning}
D.~Boscaini, J.~Masci, S.~Melzi, M.~M. Bronstein, U.~Castellani, and
  P.~Vandergheynst.
\newblock Learning class-specific descriptors for deformable shapes using
  localized spectral convolutional networks.
\newblock In {\em Computer Graphics Forum}, volume~34, pages 13--23. Wiley
  Online Library, 2015.

\bibitem{MasBosBroVan16}
D.~Boscaini, J.~Masci, E.~Rodola, and M.~M. Bronstein.
\newblock Learning shape correspondence with anisotropic convolutional neural
  networks.
\newblock In {\em Proc. NIPS}, pages 3189--3197, 2016.

\bibitem{burghard2017embedding}
O.~Burghard, A.~Dieckmann, and R.~Klein.
\newblock Embedding shapes with {G}reen's functions for global shape matching.
\newblock {\em Computers \& Graphics}, 68:1--10, 2017.

\bibitem{corman2014supervised}
E.~Corman, M.~Ovsjanikov, and A.~Chambolle.
\newblock Supervised descriptor learning for non-rigid shape matching.
\newblock In {\em Proc. ECCV Workshops (NORDIA)}, 2014.

\bibitem{cosmo2016matching}
L.~Cosmo, E.~Rodola, J.~Masci, A.~Torsello, and M.~M. Bronstein.
\newblock Matching deformable objects in clutter.
\newblock In {\em 3D Vision (3DV), 2016 Fourth International Conference on},
  pages 1--10. IEEE, 2016.

\bibitem{defferrard2016convolutional}
M.~Defferrard, X.~Bresson, and P.~Vandergheynst.
\newblock Convolutional neural networks on graphs with fast localized spectral
  filtering.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  3844--3852, 2016.

\bibitem{adam}
J.~B. D.P.~Kingma.
\newblock Adam: A method for stochastic optimization.
\newblock In {\em {ICLR}}, 2015.

\bibitem{eynard2016coupled}
D.~Eynard, E.~Rodola, K.~Glashoff, and M.~M. Bronstein.
\newblock Coupled functional maps.
\newblock In {\em 3D Vision (3DV)}, pages 399--407. IEEE, 2016.

\bibitem{ezuz2017deblurring}
D.~Ezuz and M.~Ben-Chen.
\newblock Deblurring and denoising of maps between shapes.
\newblock In {\em Computer Graphics Forum}, volume~36, pages 165--174. Wiley
  Online Library, 2017.

\bibitem{halimi2018self}
O.~Halimi, O.~Litany, E.~Rodol{`a}, A.~Bronstein, and R.~Kimmel.
\newblock Unsupervised Learning of Dense Shape Correspondence.
\newblock In {\em {CVPR}}, 2019.

\bibitem{huang2014functional}
Q.~Huang, F.~Wang, and L.~Guibas.
\newblock Functional map networks for analyzing and exploring large shape
  collections.
\newblock {\em ACM Transactions on Graphics (TOG)}, 33(4):36, 2014.

\bibitem{huang2017adjoint}
R.~Huang and M.~Ovsjanikov.
\newblock Adjoint map representation for shape analysis and matching.
\newblock In {\em Computer Graphics Forum}, volume~36, pages 151--163. Wiley
  Online Library, 2017.

\bibitem{kim11}
V.~G. Kim, Y.~Lipman, and T.~Funkhouser.
\newblock Blended intrinsic maps.
\newblock In {\em ACM Transactions on Graphics (TOG)}, volume~30, page~79. ACM,
  2011.

\bibitem{kovnatsky2015functional}
A.~Kovnatsky, M.~M. Bronstein, X.~Bresson, and P.~Vandergheynst.
\newblock Functional correspondence by matrix completion.
\newblock In {\em Proceedings of the IEEE conference on computer vision and
  pattern recognition}, pages 905--914, 2015.

\bibitem{kovnatsky2013coupled}
A.~Kovnatsky, M.~M. Bronstein, A.~M. Bronstein, K.~Glashoff, and R.~Kimmel.
\newblock Coupled quasi-harmonic bases.
\newblock In {\em Computer Graphics Forum}, volume~32, pages 439--448, 2013.

\bibitem{kovnatsky2016madmm}
A.~Kovnatsky, K.~Glashoff, and M.~M. Bronstein.
\newblock {MADMM:} a generic algorithm for non-smooth optimization on
  manifolds.
\newblock In {\em Proc. ECCV}, pages 680--696. Springer, 2016.

\bibitem{litany2017deep}
O.~Litany, T.~Remez, E.~Rodol{\`a}, A.~M. Bronstein, and M.~M. Bronstein.
\newblock Deep functional maps: Structured prediction for dense shape
  correspondence.
\newblock {\em 2017 IEEE International Conference on Computer Vision (ICCV)},
  pages 5660--5668, 2017.

\bibitem{litany2017fully}
O.~Litany, E.~Rodol{\`a}, A.~M. Bronstein, and M.~M. Bronstein.
\newblock Fully spectral partial shape matching.
\newblock In {\em Computer Graphics Forum}, volume~36, pages 247--258. Wiley
  Online Library, 2017.

\bibitem{litman2014learning}
R.~Litman and A.~M. Bronstein.
\newblock Learning spectral descriptors for deformable shape correspondence.
\newblock {\em IEEE transactions on pattern analysis and machine intelligence},
  36(1):171--180, 2014.

\bibitem{masci2015geodesic}
J.~Masci, D.~Boscaini, M.~Bronstein, and P.~Vandergheynst.
\newblock Geodesic convolutional neural networks on riemannian manifolds.
\newblock In {\em Proceedings of the IEEE international conference on computer
  vision workshops}, pages 37--45, 2015.

\bibitem{monti2017}
F.~Monti, D.~Boscaini, J.~Masci, E.~Rodol{\`{a}}, J.~Svoboda, and M.~M.
  Bronstein.
\newblock Geometric deep learning on graphs and manifolds using mixture model
  cnns.
\newblock In {\em {CVPR}}, pages 5425--5434. {IEEE} Computer Society, 2017.

\bibitem{nogneng2018improved}
D.~Nogneng, S.~Melzi, E.~Rodol{\`a}, U.~Castellani, M.~Bronstein, and
  M.~Ovsjanikov.
\newblock Improved functional mappings via product preservation.
\newblock In {\em Computer Graphics Forum}, volume~37, pages 179--190. Wiley
  Online Library, 2018.

\bibitem{nogneng2017informative}
D.~Nogneng and M.~Ovsjanikov.
\newblock Informative descriptor preservation via commutativity for shape
  matching.
\newblock {\em Computer Graphics Forum}, 36(2):259--267, 2017.

\bibitem{ovsjanikov2012functional}
M.~Ovsjanikov, M.~Ben-Chen, J.~Solomon, A.~Butscher, and L.~Guibas.
\newblock {F}unctional {M}aps: {A} {F}lexible {R}epresentation of {M}aps
  {B}etween {S}hapes.
\newblock {\em ACM Transactions on Graphics (TOG)}, 31(4):30, 2012.

\bibitem{ovsjanikov2017course}
M.~Ovsjanikov, E.~Corman, M.~Bronstein, E.~Rodol\`{a}, M.~Ben-Chen, L.~Guibas,
  F.~Chazal, and A.~Bronstein.
\newblock Computing and processing correspondences with functional maps.
\newblock In {\em ACM SIGGRAPH 2017 Courses}, SIGGRAPH '17, pages 5:1--5:62,
  2017.

\bibitem{poulenard2018topological}
A.~Poulenard, P.~Skraba, and M.~Ovsjanikov.
\newblock Topological function optimization for continuous shape matching.
\newblock In {\em Computer Graphics Forum}, volume~37, pages 13--25. Wiley
  Online Library, 2018.

\bibitem{ren2018continuous}
J.~Ren, A.~Poulenard, P.~Wonka, and M.~Ovsjanikov.
\newblock Continuous and orientation-preserving correspondences via functional
  maps.
\newblock {\em ACM Transactions on Graphics (TOG)}, 37(6), 2018.

\bibitem{rodola2017partial}
E.~Rodol{\`a}, L.~Cosmo, M.~M. Bronstein, A.~Torsello, and D.~Cremers.
\newblock Partial functional correspondence.
\newblock In {\em Computer Graphics Forum}, volume~36, pages 222--236. Wiley
  Online Library, 2017.

\bibitem{rodola-vmv15}
E.~Rodol\`{a}, M.~Moeller, and D.~Cremers.
\newblock Point-wise map recovery and refinement from functional
  correspondence.
\newblock In {\em Proc. Vision, Modeling and Visualization (VMV)}, 2015.

\bibitem{rodola2014dense}
E.~Rodol{\`a}, S.~Rota~Bulo, T.~Windheuser, M.~Vestner, and D.~Cremers.
\newblock Dense non-rigid shape correspondence using random forests.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, pages 4177--4184, 2014.

\bibitem{rosenberg1997laplacian}
S.~Rosenberg.
\newblock {\em The Laplacian on a Riemannian manifold: an introduction to
  analysis on manifolds}, volume~31.
\newblock Cambridge University Press, 1997.

\bibitem{rustamov13}
R.~Rustamov, M.~Ovsjanikov, O.~Azencot, M.~Ben-Chen, F.~Chazal, and L.~Guibas.
\newblock Map-based exploration of intrinsic shape differences and variability.
\newblock {\em ACM Trans. Graphics}, 32(4):72:1--72:12, July 2013.

\bibitem{Comp}
R.~K. Singh and J.~S. Manhas.
\newblock {\em Composition Operators on Function Spaces}.
\newblock ELSEVIER, 1993.

\bibitem{sumner2004deformation}
R.~W. Sumner and J.~Popovi{\'c}.
\newblock Deformation transfer for triangle meshes.
\newblock In {\em ACM Transactions on Graphics (TOG)}, volume~23, pages
  399--405. ACM, 2004.

\bibitem{hks}
J.~Sun, M.~Ovsjanikov, and L.~Guibas.
\newblock A {C}oncise and {P}rovably {I}nformative {M}ulti-{S}cale {S}ignature
  {B}ased on {H}eat {D}iffusion.
\newblock In {\em Computer graphics forum}, volume~28, pages 1383--1392, 2009.

\bibitem{tam2013registration}
G.~K. Tam, Z.-Q. Cheng, Y.-K. Lai, F.~C. Langbein, Y.~Liu, D.~Marshall, R.~R.
  Martin, X.-F. Sun, and P.~L. Rosin.
\newblock Registration of 3d point clouds and meshes: a survey from rigid to
  nonrigid.
\newblock {\em IEEE transactions on visualization and computer graphics},
  19(7):1199--1217, 2013.

\bibitem{shot}
F.~Tombari, S.~Salti, and L.~Di~Stefano.
\newblock Unique signatures of histograms for local surface description.
\newblock In {\em International Conference on Computer Vision (ICCV)}, pages
  356--369, 2010.

\bibitem{van2011survey}
O.~Van~Kaick, H.~Zhang, G.~Hamarneh, and D.~Cohen-Or.
\newblock A survey on shape correspondence.
\newblock In {\em Computer Graphics Forum}, volume~30, pages 1681--1707, 2011.

\bibitem{vestnerefficient}
M.~Vestner, Z.~L{\"a}hner, A.~Boyarski, O.~Litany, R.~Slossberg, T.~Remez,
  E.~Rodola, A.~Bronstein, M.~Bronstein, R.~Kimmel, and D.~Cremers.
\newblock Efficient deformable shape correspondence via kernel matching.
\newblock In {\em Proc. 3DV}, 2017.

\bibitem{vestner2017product}
M.~Vestner, R.~Litman, E.~Rodol{\`a}, A.~Bronstein, and D.~Cremers.
\newblock Product manifold filter: Non-rigid shape correspondence via kernel
  density estimation in the product space.
\newblock In {\em Proc. CVPR}, pages 6681--6690, 2017.

\bibitem{wang2018kernel}
L.~Wang, A.~Gehre, M.~M. Bronstein, and J.~Solomon.
\newblock Kernel functional maps.
\newblock In {\em Computer Graphics Forum}, volume~37, pages 27--36. Wiley
  Online Library, 2018.

\bibitem{wang2018vector}
Y.~Wang, B.~Liu, K.~Zhou, and Y.~Tong.
\newblock Vector field map representation for near conformal surface
  correspondence.
\newblock In {\em Computer Graphics Forum}, volume~37, pages 72--83. Wiley
  Online Library, 2018.

\bibitem{wei2016dense}
L.~Wei, Q.~Huang, D.~Ceylan, E.~Vouga, and H.~Li.
\newblock Dense human body correspondences using convolutional networks.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and
  Pattern Recognition}, pages 1544--1553, 2016.

\bibitem{yan2014low}
D.-M. Yan, G.~Bao, X.~Zhang, and P.~Wonka.
\newblock Low-resolution remeshing using the localized restricted voronoi
  diagram.
\newblock {\em IEEE transactions on visualization and computer graphics},
  20(10):1418--1427, 2014.

\end{thebibliography}

